Persona-aware Generative Model for Code-mixed Language

Code-mixing and script-mixing are prevalent across online social networks and multilingual societies. However, a user's preference toward code-mixing depends on the socioeconomic status, demographics of the user, and the local context, which existing generative models mostly ignore while generating code-mixed texts. In this work, we make a pioneering attempt to develop a persona-aware generative model to generate texts resembling real-life code-mixed texts of individuals. We propose a Persona-aware Generative Model for Code-mixed Generation, PARADOX, a novel Transformer-based encoder-decoder model that encodes an utterance conditioned on a user's persona and generates code-mixed texts without monolingual reference data. We propose an alignment module that re-calibrates the generated sequence to resemble real-life code-mixed texts. PARADOX generates code-mixed texts that are semantically more meaningful and linguistically more valid. To evaluate the personification capabilities of PARADOX, we propose four new metrics -- CM BLEU, CM Rouge-1, CM Rouge-L and CM KS. On average, PARADOX achieves 1.6 points better CM BLEU, 47% better perplexity and 32% better semantic coherence than the non-persona-based counterparts.

==> tables/main_results.tex <==
\begin{table*}[t]
\centering
\scalebox{0.4}{
{\begin{tabular}{lrrrrrrrr}
\toprule
\textbf{Model} &\multicolumn{2}{c}{\textbf{CM BLEU} $\uparrow$} &\multicolumn{2}{c}{\textbf{CM Rouge-1} $\uparrow$} &\multicolumn{2}{c}{\textbf{CM Rouge-L} $\uparrow$} &\multicolumn{2}{c}{\textbf{CM KS} $\downarrow$} \\\cmidrule{2-9}
\textbf{} &\textbf{Twitter} &\textbf{YouTube} &\textbf{Twitter} &\textbf{YouTube} &\textbf{Twitter} &\textbf{YouTube} &\textbf{Twitter} & \textbf{YouTube} \\\midrule

Transformer & 22.21 & 29.36 & 58.69 & 61.02 & 51.10 & 57.27 & 0.42 & 0.37 \\
\hline
\rowcolor{maroon!10}  {\modelname} & 23.64 & 29.02 & 59.71 & 61.62 & 52.24 & 57.83 & 0.36 & \textbf{0.34} \\
\hdashline
\rowcolor{maroon!10}  (-) Contextual Persona & \textbf{24.06} & \textbf{30.67} & \textbf{60.03} & \textbf{62.44} & \textbf{52.52} & \textbf{58.71} & 0.35 & \textbf{0.34}  \\
\rowcolor{maroon!10}  (-) Alignment & 23.56 & \textbf{30.67} & 59.84 & 62.12 & 52.22 & 58.43 & \textbf{0.32} & 0.37 \\
\rowcolor{maroon!10}  (-) FAME & 20.37 & 29.36 & 55.78 & 60.80 & 49.16 & 57.37 & 0.36 & 0.37 \\
\bottomrule
\end{tabular}
}}
\caption{Extrinsic evaluation of Transformer and {\modelname} in terms of preserving user-level switching patterns ($\uparrow$ ({\em resp.} $\downarrow$): higher ({\em resp.} lower) value indicates better performance).}
\label{tab:main_result}
\end{table*}

==> tables/more_examples.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.75}{
\begin{tabular}{c| p{16em}| c | c}
\hline
Model & Generated Text & Semantic Coherence & Linguistic Quality\\
\hline
\multirow{4}{*}{\modelname} & \textbf{CM:} are bhai apne! & 3.70 & 3.60\\
& \textbf{Eng:} Hey my brother! & & \\
\cdashline{2-4}
%& \textbf{CM:} school ka time ho raha hai bhai maine time & \multirow{2}{*}{3.20} & \multirow{2}{*}{3.27}\\
%& \textbf{Eng:} It's school time brother, I have time & & \\
& \textbf{CM:} bhai bahut thik ho gaya & 4.27 & 4.27 \\
& \textbf{Eng:} brother is very well & & \\
\hline
%\multirow{6}{*}{Transformer} & \textbf{CM:} dard bhai yahi nhi hai.. & 3.80 & 3.57 \\
%& \textbf{Eng:} This is not the pain brother.. & & \\
%\hdashline
\multirow{4}{*}{Transformer} & \textbf{CM:} rockstar walo se samjha media........ & 3.07 & 3.57\\
& \textbf{Eng:} Media understood by rockstars & & \\
\cdashline{2-4}
& \textbf{CM:} boy likha hai thanks bhai & 3.57 & 3.53 \\
& \textbf{Eng:} Boy has written thanks brother & & \\
\hline
\end{tabular}}
\caption{Examples of code-mixed texts generated by {\modelname} and Transformer with human annotated average Semantic coherence and linguistic quality scores.} \label{tab:few_more_examples}
\end{table*}

==> tables/optimizers.tex <==
\begin{table*}[!t]\centering
\scalebox{0.8}{
\begin{tabular}{c c c c c c c}
\hline
Model & Training Curriculum & Training Step & Optimizer & Learning rate & $\beta_1$ & $\beta_2$ \\\midrule
%Transformer & Vanilla & - & Adam & 4e-4 & 0.9 & 0.98 \\
\hline
%Transformer & Distillation & - & Adam & 4e-4 & 0.9 & 0.98 \\
%\hline
%Transformer:Student & \multirow{3}{*}{Meta Distillation} & Student evaluation & SGD & 4e-4 & - & -\\
%Transformer:Teacher & & Teacher alignment & SGD & 4e-5 & - & -\\
%Transformer:Student & & Student relearning & Adam & 4e-4 & 0.9 & 0.98 \\
%\hline
{\modelname} & Vanilla & - & Adam & 4e-4 & 0.9 & 0.98 \\
\hline
{\modelname} & Distillation & - & Adam & 4e-4 & 0.9 & 0.98 \\
\hline
{\modelname}:Student & \multirow{3}{*}{Meta Distillation} & Student evaluation & SGD & 4e-4 & - & -\\
{\modelname}:Teacher & & Teacher alignment & SGD & 4e-5 & - & -\\
{\modelname}:Student & & Student relearning & Adam & 4e-4 & 0.9 & 0.98 \\

\hline
\end{tabular}
}
\caption{Optimizers for different models used for training.} \label{tab:optimizer}
\end{table*}

==> tables/user_results.tex <==
\begin{table}[!htp]\centering
\scalebox{1.5}{
\begin{tabular}{lrrrr}\toprule
\textbf{Model} &\multicolumn{2}{c}{\textbf{CS KS} $\downarrow$} &\multicolumn{2}{c}{\textbf{MSD} $\downarrow$} \\\cmidrule{2-5}
\textbf{} &\textbf{Twitter} &\textbf{YouTube} &\textbf{Twitter} &\textbf{YouTube} \\
\hline
%Transformer & 0.268 ($\pm$ 0.017) & 0.257 ($\pm$ 0.010) & 0.363 ($\pm$ 0.013) & 0.319 ($\pm$ 0.004)\\
Transformer & 0.42 & 0.37 & 6.52\% & 5.15\%\\
\hline
\rowcolor{maroon!10} {\modelname} & 0.36 & \textbf{0.34} & 5.66\% & \textbf{4.91\%}\\
\hdashline
\rowcolor{maroon!10}(-) Contextual Persona & 0.35 & \textbf{0.34} & 5.45\% & \textbf{4.91\%}\\
\rowcolor{maroon!10} (-) Alignment & \textbf{0.32} & 0.37 & \textbf{5.30\%} & 5.14\%\\
%\rowcolor{maroon!20} (-) User Persona \\
\rowcolor{maroon!10} (-) FAME & 0.36 & 0.37 & 6.34\% & 5.33\%\\
\bottomrule
\end{tabular}
}
\caption{Kolmogorov-Smirnov distance between generated and original CMI distribution of users on generation. Lower KS distance signifies better personalization capability of the generative models.}\label{tab:user_result}
%For all the metrics, a lower value indicates better generability of models. 
\end{table}
